Variational Schr\"odinger Momentum Diffusion

The momentum Schr\"odinger Bridge (mSB) has emerged as a leading method for accelerating generative diffusion processes and reducing transport costs. However, the lack of simulation-free properties inevitably results in high training costs and affects scalability. To obtain a trade-off between transport properties and scalability, we introduce variational Schr\"odinger momentum diffusion (VSMD), which employs linearized forward score functions (variational scores) to eliminate the dependence on simulated forward trajectories. Our approach leverages a multivariate diffusion process with adaptively transport-optimized variational scores. Additionally, we apply a critical-damping transform to stabilize training by removing the need for score estimations for both velocity and samples. Theoretically, we prove the convergence of samples generated with optimal variational scores and momentum diffusion. Empirical results demonstrate that VSMD efficiently generates anisotropic shapes while maintaining transport efficacy, outperforming overdamped alternatives, and avoiding complex denoising processes. Our approach also scales effectively to real-world data, achieving competitive results in time series and image generation.

==> chapters/diagrams_comparison.tex <==

\tikzset{font=\scriptsize,
edge from parent fork down,
level distance=1.3cm, align=center,
every node/.style=
    {top color=white,
    bottom color=blue!5,
    rectangle,rounded corners,
    minimum height=6mm,
    draw=blue!10,
    % very thick,
    drop shadow,
    align=center,
    text depth = 0pt
    },
edge from parent/.style=
    {draw=blue!30,
    thick,
    }}

% \begin{tikzpicture}
% \Tree 
% [.{More Transport Efficiency}
%         [.{SGM \citep{score_sde}}
%             [.{CLD \citep{CLD}}
%                 [.{ Linear forward process \\ Univariate \\ \textcolor{darkgreen}{Simulation-free}}
%                     [.{\textcolor{red}{Backward process} \\ \textcolor{red}{Simulation-based}}
%                             [.{\textcolor{red}{Isotropic Generation}}
%                                 [.{\textcolor{darkgreen}{Training loss: L2}}
%                                     [.{\textcolor{red}{No optimal transport}}
%                                         ]
%                                 ]
%                             ]
%                     ]
%                 ]
%             ]
%         ]
%         [.{VSDM \citep{VSDM}}
%             [.{\textbf{VSMD (this work)} }
%                 [.{ Linear forward process \\ Multivariate \\ \textcolor{darkgreen}{Simulation-free}}
%                     [.{\textcolor{red}{Simulation-based}}
%                             [.{\textcolor{darkgreen}{Anisotropic Generation}}
%                                 [.{\textcolor{darkgreen}{L2}/ \textcolor{red}{Divergence}}
%                                     [.{\textcolor{darkgreen}{Suboptimal transport}}
%                                         ]
%                                 ]
%                             ]
%                     ]
%                 ]
%             ]
%         ]
%         [.{SB \citep{forward_backward_SDE}}
%             [.{mSB \citep{mSB}}
%                 [.{Nonlinear forward process \\ \textcolor{red}{Simulation-based}}
%                     [.{\textcolor{red}{Simulation-based}}
%                             [.{\textcolor{darkgreen}{Anisotropic Generation}}
%                                 [.{\textcolor{red}{Divergence/ Divergence}}
%                                     [.{\textcolor{darkgreen}{Optimal transport}}
%                                         ]
%                                 ]
%                             ]
%                     ]
%                 ]
%             ]
%         ]
% ]
% \end{tikzpicture}



\begin{tikzpicture}
\Tree 
[.{More Transport Efficiency}
        [.{SGM \citep{score_sde}}
            [.{CLD \citep{CLD}}
                [.{ Linear forward process \\ Univariate \\ \textcolor{darkgreen}{Simulation-free}}
                            [.{\textcolor{red}{Isotropic Generation}}
                                [.{\textcolor{darkgreen}{Training loss: L2}}
                                    [.{\textcolor{red}{No optimal transport}}
                                        ]
                                ]
                            ]
                ]
            ]
        ]
        [.{VSDM \citep{VSDM}}
            [.{\textbf{VSMD (this work)} }
                [.{ Linear forward process \\ Multivariate \\ \textcolor{darkgreen}{Simulation-free}}
                            [.{\textcolor{darkgreen}{Anisotropic Generation}}
                                [.{\textcolor{darkgreen}{L2}/ \textcolor{red}{Divergence}}
                                    [.{\textcolor{darkgreen}{Suboptimal transport}}
                                        ]
                                ]
                            ]
                ]
            ]
        ]
        [.{SB \citep{forward_backward_SDE}}
            [.{mSB \citep{mSB}}
                [.{Nonlinear forward process \\ \textcolor{red}{Simulation-based}}
                            [.{\textcolor{darkgreen}{Anisotropic Generation}}
                                [.{\textcolor{red}{Divergence/ Divergence}}
                                    [.{\textcolor{darkgreen}{Optimal transport}}
                                        ]
                                ]
                            ]
                ]
            ]
        ]
]
\end{tikzpicture}





% \begin{table*}
% \begin{tabular}{ c | c | c | c }
% \hline
% Properties & SGM \scriptsize{\citep{score_sde}} & SB \scriptsize{\citep{forward_backward_SDE}} & VSDM \citep{VSDM} \\ 
% Properties & CLD \scriptsize{\citep{CLD}} & mSB \scriptsize{\citep{mSB}} & VSMD (ours) \\ 
% \hline
% Forward Process & Univariate &  Nonlinear  & Multivariate \\ 
% \hline
% Optimal Transport & $\color{red}\times$  &  \textcolor{darkgreen}{Optimal}  &  \textcolor{darkgreen}{Sub-Optimal} \\ 
% \hline
% Simulation-Free Forward Process &  \color{darkgreen}\checkmark  &  $\color{red}\times$ &  \color{darkgreen}\checkmark   \\
% \hline
% Simulation-Free Backward Process & N/A  &  $\color{red}\times$ &  $\color{red}\times$  \\
% \hline
% Training Losses &  \textcolor{darkgreen}{L2}  &  \footnotesize{\textcolor{red}{Divergence/ Divergence}} &  \textcolor{darkgreen}{L2}/ \textcolor{red}{Divergence}  \\
% \hline
% Anisotropic Generation & $\color{red}\times$  & \color{darkgreen}\checkmark  &  \color{darkgreen}\checkmark \\ 
% \hline
% \end{tabular}
% \end{table*}


==> chapters/proof_critical_damped.tex <==

\subsection{Diagonal Time Invariant Simplification}

We begin by writing the forward process, we write $\bA_{xt} = \alpha$ and $\bA_{vt} = \beta$ then the forward process on a per coordiante basis writes:

\begin{align}
d\bx_t &= \frac{1}{2} \beta_t \bv_t \\
d\bv_t &= \frac{-1}{2} \beta_t (\bx_t + \gamma \bv_t - 2 \gamma \alpha \bx_t - 2\gamma \beta \bv_t) + \sqrt{\gamma \beta_t} d \bw_t\\
&= \frac{-1}{2} \beta_t ((1-2 \gamma \alpha) \bx_t + (\gamma - 2\gamma \beta )\bv_t) + \sqrt{\gamma \beta_t} d \bw_t\\
&= \frac{-1}{2} \beta_t (\omega_0^2 \bx_t + \tilde{\gamma} \bv_t) + \sqrt{\gamma \beta_t} d \bw_t
\end{align}\label{FB-SDE-linear}

Then in order  to have optimal damping we require that $2\omega_0 = \tilde{\gamma}$ \Kevin{You're right it was a typo, I corrected it} or equivalently we need:
\[ 2\sqrt{(1-2 \gamma \alpha)} = (\gamma - 2\gamma \beta ) \]

Which implies that:
\[\beta = \frac{1}{2} - \frac{1}{\gamma}\sqrt{(1-2 \gamma \alpha)} \]

where $\bA_{xt}$ and $\bA_{vt}$ are $d\times d$ matrices to be optimized.

\Wei{underdamped example $N\omega_0^2 = \tilde{\gamma}^2$}

\Wei{\[ \sqrt{N}\sqrt{(1-2 \gamma \alpha)} = (\gamma - 2\gamma \beta ) \]}
\Wei{\[\beta = \frac{1}{2} - \frac{\sqrt{N}}{2\gamma}\sqrt{(1-2 \gamma \alpha)} \]}


% \Wei{I found empirically \[\beta = \frac{1}{4} - \frac{1}{2\gamma}\sqrt{(1-4 \gamma \alpha)} \] works better}

% \Wei{$$d\bv_t = \frac{-1}{2} \beta_t (\bx_t + \gamma \bv_t - 4 \gamma \alpha \bx_t - 4\gamma \beta \bv_t) + \sqrt{\gamma \beta_t} d \bw_t$$}

If we add a mass variable to our problem as done in CLD then it rewrites as: 

\begin{align}
d\bx_t &= \frac{1}{2} \beta_t M^{-1} \bv_t \\
d\bv_t &= \frac{-1}{2} \beta_t (\omega_0^2 \bx_t + \tilde{\gamma} M^{-1} \bv_t) + \sqrt{\gamma \beta_t} d \bw_t
\end{align}\label{FB-SDE-linear}

If we then apply a change of variables $\tilde{\bv_t} = M^{-1} \bv_t$ and apply Ito's Lemma we get the system (I dropped the tilde for notation simplicity), also for simplicity let $\beta_t = 2$ (since this is just a time reparametrization it doesn't change anything):

\begin{align}
d\bx_t &= \bv_t \\
d\bv_t &= -M^{-1} \omega_0^2 \bx_t - \tilde{\gamma} M^{-1} \bv_t dt + M^{-1} \sqrt{2\gamma} d \bw_t
\end{align}\label{FB-SDE-linear}

We can rewrite this as:

\[\ddot{\bx_t} = -M^{-1} \omega_0^2 \bx_t - \tilde{\gamma} M^{-1} \dot{\bx_t} + M^{-1} \sqrt{\gamma \beta_t} d \bw_t \]

Or equivalently:

\[\ddot{\bx_t} + \tilde{\gamma} M^{-1} \dot{\bx_t} + M^{-1} \omega_0^2 \bx_t - M^{-1} \sqrt{\gamma \beta_t} d \bw_t =0 \]

This is the part that is a little weird, but shouldn't be too hard to derive  in the general case. In the book they derive the critical damping for the ODE case. So they look at:
\[\ddot{\bx_t} + \tilde{\gamma} M^{-1} \dot{\bx_t} + M^{-1} \omega_0^2 \bx_t = 0\]

If we write this in matrix form again it is something like:
\begin{align}
d\begin{pmatrix}
 \bx_t   \\
 \bv_t
\end{pmatrix}
&= 
\begin{pmatrix}
    0 & 1 \\
    -M^{-1} \omega_0^2 & - \tilde{\gamma} M^{-1}
\end{pmatrix}
\begin{pmatrix}
 \bx_t   \\
 \bv_t
\end{pmatrix}
\end{align}

The eigenvalues of this matrix are given by:
\[\lambda_{\pm} = \frac{- \tilde{\gamma} M^{-1} \pm \sqrt{\tilde{\gamma}^2 M^{-2} - 4 M^{-1} \omega_0^2}}{2}\]

The critical damping occurs in the case where $\tilde{\gamma}^2 M^{-2} = 4 M^{-1} \omega_0^2$ or equivalently:
\[\tilde{\gamma}^2= 4 M \omega_0^2\]


\label{FB-SDE-linear}

==> chapters/proof_diagonal.tex <==

\section{Proof for Overdamped Case}

Given a forward process: 

\[dX_t = -\frac{-\beta_t}{2} D_tx_t dt + \sqrt{\beta_t} dt\]

Where $X_0\in\R^d$ and $D_t \in \R^{d\times d}$ and assume that $D$ is symmetric. Then we know by a similar argument as above that:

    
\[X_t =e^{-\frac{1}{2} [\beta\bD]_t} \bx_0 + C_tH_t^{-1} z\]

\Wei{should be \[X_t =e^{-\frac{1}{2} [\beta\bD]_t} \bx_0 + L_t z\], where $L L^{\intercal} =  C_tH_t^{-1}?$}

Where:
\begin{align}\label{cov_dynamics}
  \begin{pmatrix}
    \bC_t \\
    \bH_t
  \end{pmatrix} &=
  \exp\Bigg[
  \begin{pmatrix}
    -\frac{1}{2}[\beta\bD]_t & \big[\beta \bm{\mathrm{I}}_{d}\big]_t \\
    \bm{0} &  \frac{1}{2}[\beta\bD^{\intercal}]_t
  \end{pmatrix}
  \Bigg]
        \begin{pmatrix}
          {\bSigma}_0 \\
          {\bI_{2d}} 
        \end{pmatrix},            
\end{align}

Additionally it is well known that (for instance see \cite{dieci2001conditioning}) that if:
\[
A = \begin{pmatrix}
    A_{11} & A_{12} \\
    0 & A_{22}
\end{pmatrix}
\]
Then:
\[e^A = \begin{pmatrix}
    e^{A_{11}} & \int_0^1 e^{A_{11}(1-s)} A_{12} e^{A_{22}s}ds \\
    0 & e^{A_{22}}
\end{pmatrix}
\]


So in our case this means that:
\begin{align}\label{cov_dynamics}
  \begin{pmatrix}
    \bC_t \\
    \bH_t
  \end{pmatrix} &=
  \exp\Bigg[
  \begin{pmatrix}
    \exp(-\frac{1}{2}[\beta\bD]_t) & \int_0^1 \exp(-\frac{1}{2}[\beta\bD]_t (1-s)) \big[\beta \bm{\mathrm{I}}_{d}\big]_t \exp(\frac{1}{2}[\beta\bD^{\intercal}]_t s \text{\Wei{some $s$ term?}\Kevin{added}}) \\
    \bm{0} &  \exp(\frac{1}{2}[\beta\bD^{\intercal}]_t)
  \end{pmatrix}
  \Bigg]
        \begin{pmatrix}
          0 \\
          {\bI_{2d}} 
        \end{pmatrix},            
\end{align}

Now let me focus on the big term:
\begin{align*}
C_t &= \int_0^1 \exp(-\frac{1}{2}[\beta\bD]_t (1-s)) \big[\beta \bm{\mathrm{I}}_{d}\big]_t \exp(\frac{1}{2}[\beta\bD^{\intercal}]_t s) \\
&=  
\big[\beta\big]_t \int_0^1 \exp(-\frac{1}{2}[\beta\bD]_t (1-s)) \exp(\frac{1}{2}[\beta\bD^{\intercal}]_t s) \\
&=  
\big[\beta\big]_t \int_0^1 \exp([\beta\bD]_t (s-1/2)) ds \\
&=  
\big[\beta\big]_t \exp(-\frac{1}{2}[\beta\bD]_t)) \int_0^1 \exp([\beta\bD]_t s) ds \\
&=  
\big[\beta\big]_t \exp(-\frac{1}{2}[\beta\bD]_t)) (\exp([\beta\bD]_t) - I) \big[\beta D]_t^{-1} 
\end{align*}

Since $H_t^{-1} = \exp(-\frac{1}{2}[\beta\bD]_t)$ then we have that:

\begin{align*}
C_tH_t^{-1} &= 
\big[\beta\big]_t \exp(-\frac{1}{2}[\beta\bD]_t)) (\exp([\beta\bD]_t) - I) \big[\beta D]_t^{-1} \exp(-\frac{1}{2}[\beta\bD]_t)
\end{align*}
Notice that $[\beta D]^{-1}$ and $\exp(-.5 [\beta D]_t)$ conmute because they are simultaneously diagonalizable. So that we can change this to:
\begin{align*}
C_tH_t^{-1} &= 
\big[\beta\big]_t \exp(-\frac{1}{2}[\beta\bD]_t)) (\exp([\beta\bD]_t) - I) \big[\beta D]_t^{-1} \exp(-\frac{1}{2}[\beta\bD]_t) \\
&= 
\big[\beta\big]_t (I - \exp(-\frac{1}{2}[\beta\bD]_t)) \big[\beta D]_t^{-1} 
\end{align*}
Now recall that:
\[X_t =e^{-\frac{1}{2} [\beta\bD]_t} \bx_0 + C_tH_t^{-1} z\]
So for $X_t \to \mathcal{N}(0,I)$ we need two things:
\begin{enumerate}
    \item $e^{-\frac{1}{2} [\beta\bD]_t} \to 0$
    \item $C_tH_t{-1} \to I$
\end{enumerate}
Then:
\begin{align*}
C_tH_t^{-1} &= 
\big[\beta\big]_t (I - \exp(-\frac{1}{2}[\beta\bD]_t)) \big[\beta D]_t^{-1}
\\
&\to \lim_{t\to \infty} \big[\beta\big]_t \big[\beta D]_t^{-1} \\
&= I
\end{align*}
So for the last convergence to happen, we can equivalently require that $[\beta D]_t [\beta]_t^{-1} \to I $ therefore if we analyze coordinate by coordinate of $D$ we are requiring that:
\begin{enumerate}
    \item $[\beta]_t^{-1}[\beta D_{ij}]_t \to 0$
    \item $[\beta D_{ii}]_t \to [\beta]_t$
\end{enumerate}

Which implies that $D_{ij} = o(1)$



==> main_modules.tex <==

\Wei{Wei's remark}

\Kevin{Kevin's remark}
\begin{itemize}
    \item Critically damped diffusion
    \item multivariate diffusion.
\end{itemize}



TO DO LIST IN EXPERIMENTS

\begin{itemize}
    \item generation of anisotropic shapes \Wei{done}
    \teim generation of straighter paths or is faster than VSDM or different damping or visualize both x and v? \Wei{to do}

    \item time series (\Wei{prepare script for tuning})
    \item image generation (\Wei{either standard generation or conditional ones})
\end{itemize}


TO DO LIST IN THEORY 

\begin{itemize}
    \item derive critical-damped rules
    \item generation quality following \url{https://arxiv.org/pdf/2209.11215}
\end{itemize}

\section{Introduction}


\section{Methodology}

\paragraph{Notations:} We denote the augmented variable by $\ba:=(\bx, \bv)^\intercal \in \mathrm{R}^{2d}$, where $\bx\in\mathrm{R}^{d}$ is the data and $\bv\in \mathrm{R}^{d}$ is the velocity. We denote $\beta_t:=\beta(t)$.




\subsection{Forward-Backward SDE with Momentum}

\subsection{From Schr\"{o}dinger Bridge problem (SBP) to FB-SDE}
\label{Preliminaries_SBP}

\input{./chapters/method.tex}

\section{Theory}

\input{./chapters/proof_critical_damped.tex}

\section{Experiments}

\subsection{Diagonal Time Invariant Simplification}


\subsection{Simulation-Free Expression of Backward Score}

\subsection{Adaptive optimize the approximation}
Assume a prior knowledge of 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

